Offline Meta Reinforcement Learning with In-Distribution Online Adaptation

Recent offline meta-reinforcement learning (meta-RL) methods typically utilize task-dependent behavior policies (e.g., training RL agents on each individual task) to collect a multi-task dataset. However, these methods always require extra information for fast adaptation, such as offline context for testing tasks. To address this problem, we first formally characterize a unique challenge in offline meta-RL: transition-reward distribution shift between offline datasets and online adaptation. Our theory finds that out-of-distribution adaptation episodes may lead to unreliable policy evaluation and that online adaptation with in-distribution episodes can ensure adaptation performance guarantee. Based on these theoretical insights, we propose a novel adaptation framework, called In-Distribution online Adaptation with uncertainty Quantification (IDAQ), which generates in-distribution context using a given uncertainty quantification and performs effective task belief inference to address new tasks. We find a return-based uncertainty quantification for IDAQ that performs effectively. Experiments show that IDAQ achieves state-of-the-art performance on the Meta-World ML1 benchmark compared to baselines with/without offline adaptation.

==> 1-Introduction-bak.tex <==
\vspace{-0.2in}
\section{Introduction}

Human intelligence is capable of learning a wide variety of skills from past history and can adapt to new environments by transferring skills within limited experience. Current reinforcement learning (RL) has surpassed human-level performance \citep{mnih2015human,silver2017mastering,hafner2019dream} by requiring a large amount of experience. However, in many real-world applications, RL encounters two challenges of multiple tasks and costly online interactions. In multi-task settings, such as robotic manipulation or locomotion \citep{yu2020meta}, agents are expected to solve new tasks with few-shot adaptation after learning on individual tasks shared with common structures. Moreover, collecting sufficient exploratory interactions is usually expensive or dangerous in robotics \citep{rafailov2021offline}, autonomous driving \citep{yu2018bdd100k}, and healthcare \citep{gottesman2019guidelines}. One popular paradigm for breaking this practical barrier is \textit{offline meta reinforcement learning} \citep[offline meta-RL;][]{li2020focal,mitchell2021offline}, which trains a meta-RL agent with pre-collected offline multi-task datasets and enables fast policy adaptation to unseen tasks.

Recent offline meta-RL methods \citep{li2020focal,mitchell2021offline,dorfman2021offline} typically collect a multi-task dataset with task-dependent behavior policies, which is naturally applicable to big data in practical applications \citep{levine2020offline}. They always train a bunch of behavior RL agents on different tasks and combine the individual datasets into an overall dataset. However, these offline meta-RL approaches always require additional information for fast adaptation. For example, FOCAL \citep{li2020focal} and MACAW \citep{mitchell2021offline} conduct offline adaptation, in which offline contexts are available in the unseen tasks. BORel \citep{dorfman2021offline} and SMAC \citep{pong2022offline} employ few-shot online adaptation, but the former assumes a known reward function, and the later requires free interactions with the environment without reward supervision. Therefore, achieving effective few-shot online adaptation remains an open problem for offline meta-RL.

\begin{figure}
	\centering
	\vspace{-0.3in}
	\includegraphics[width=\linewidth]{figures/motivation.pdf}
	\caption{Illustration of data distribution mismatch between offline training and online adaptation.}
	\label{fig:motivation}
	\vspace{-0.3in}
\end{figure}

One particular challenge of meta-RL compared to meta-supervised learning is the need to learn how to explore in the testing environments \citep{finn2019meta,zhang2021metacure}. In offline meta-RL, the gap of reward and transition functions between offline training and online adaptation presents a unique conundrum for meta-policy learning, namely \textbf{\textit{data distribution mismatch}}. As shown in Figure \ref{fig:motivation}, when we collect an offline dataset using the expert policy for each task, the robot will be meta-trained on all {\color{napiergreen}\textbf{successful trajectories}} (\imgintext{figures/x2.png}). The robot will fast explore the environment to reduce task uncertainty in meta-testing. However, when it tries the middle path and hits a stone, this {\color{blue-violet}\textbf{failed adaptation trajectory}} (\imgintext{figures/x1.png}) does not match the training data distribution. Where should the robot go in the second trial? To build a theory to study this phenomenon, we utilize the perspective of Bayesian RL \citep[BRL;][]{duff2002optimal,zintgraf2019varibad,dorfman2021offline}, which maintains a task belief given the context history and learns a meta-policy on the belief states. Our theoretical analysis shows that task-dependent data collection results in an inconsistency between offline meta-policy evaluation and online adaptation evaluation, which contrasts with policy evaluation consistency in offline single-task RL \citep{fujimoto2019off}. To bridge this gap, we introduce a new mechanism of data distribution correction that incorporates additional information about task-dependent behavior policies into overall beliefs. This mechanism aligns the data distribution and provides the consistency of policy evaluation by requiring the agent to filter out out-of-distribution episodes. 

In practice, detecting whether an adaptation episode is in the distribution of the training dataset is challenging \citep{yu2021combo,wang2021offline}. To support our theoretical implications in practical realization, we adopt a common heuristic of offline RL \citep{fujimoto2019off,kostrikov2021offline}, \ie{}, out-of-distribution data cannot perform well, and propose a novel online adaptation approach, called \textit{\textbf{G}reedy \textbf{C}ontext-based data distribution \textbf{C}orrection} (GCC). GCC is a context-based meta-RL algorithm \citep{rakelly2019efficient} to maximize the final performance in online adaptation, which extracts a task belief from prior experience, samples “task hypotheses”, tries these trials, and updates the posterior belief in a closed loop. To align adaptation context into the meta-training distribution, GCC utilizes greedy task inference, which diversely samples “task hypotheses” and selects a hypothesis with the highest return to update the belief. For example in Figure \ref{fig:motivation}, the robot will try other paths and the failed adaptation trajectory (middle) will not be used for task inference because it is out-of-distribution with lower return. To our best knowledge, our method is the first to design a delicate context mechanism to achieve effective online adaptation for offline meta-RL and has the advantage of directly combining with off-the-shelf context-based offline meta-training algorithms (\eg{}, FOCAL \citep{li2020focal}). Such a selective context structure shares similar motivations with human perception and memory. Studies from Psychology \citep{huang2009task} show that, selective attention protects cognition and decision-making from intrusions of target-irrelevant stimulus attributes.

Our main contribution is to formalize a specific challenge (\ie{}, data distribution mismatch) in offline meta-RL with online adaptation and propose a greedy context mechanism with theoretical motivation. We evaluate the performance of GCC in several didactic problems proposed by prior work \citep{rakelly2019efficient,li2020focal} and Meta-World ML1 benchmark with 50 tasks \citep{yu2020meta}. In these didactic problems, GCC demonstrates that our delicate context mechanism can accurately infer correct task identification, whereas the original online adaptation methods will suffer due to out-of-distribution data. Empirical results on more challenging Meta-World ML1 benchmark show that GCC significantly outperforms baselines with few-shot online adaptation. GCC also achieves better or comparable performance than baselines with offline adaptation, suggesting that offline context may not be necessary in the testing environments.


==> 5-IDAQ.tex <==
\vspace{-0.1in}
\section{IDAQ: In-Distribution Online Adaptation with Uncertainty Quantification}

In this section, we will investigate a practical scheme to address transition-reward distribution shift in offline meta-RL. Inspired by the theory in Section~\ref{sec:theory}, we aim to \textbf{\textit{distinguish}} whether an adaptation episode is in the distribution of the offline dataset, and utilize meta-policies with Thompson sampling \citep{strens2000bayesian} to generate in-distribution online adaptation. Therefore, we will introduce a novel context-based online adaptation algorithm, called \textit{\textbf{I}n-\textbf{D}istribution online \textbf{A}daptation with uncertainty \textbf{Q}uantification} (IDAQ), which infers in-distribution context for solving meta-testing tasks. IDAQ consists of three main components: (i) an off-the-shelf context-based offline meta-training method, (ii) an in-distribution online adaptation framework, and (iii) a plug-in uncertainty quantification function.

\vspace{-0.1in}
\subsection{In-Distribution Online Adaptation Algorithm}

To support effective offline meta-training, we employ a state-of-the-art off-the-shelf context-based algorithm $\sA$, i.e., FOCAL \citep{li2020focal}, which follows the learning paradigm of latent task embedding (see Section \ref{sec:task-embedding}). During online meta-testing, our adaptation protocol adopts the popular framework of \textit{Thompson sampling} \citep{rakelly2019efficient}. IDAQ will iteratively update posterior task belief based on online interactions with environment and execute the meta-policy with a sampled "task hypothesis".
%This adaptation paradigm is generalized from Bayesian inference \citep{thompson1933likelihood} and has a solid background in RL theory \citep{agrawal2012analysis}. 

For in-distribution online adaptation, IDAQ utilizes a given uncertainty quantification $\sQ(\tau)$ to empirically measure the confidence that online experience $\{\tau_i\}$ are in-distribution. Note that the context encoder $q(z|\bm{c})$ (i.e., a task inference module) is meta-trained in the offline dataset and cannot handle out-of-distribution adaptation \citep{mendonca2020meta}, where $\bm{c}$ is the episode-based context. To realize reliable task belief updating, IDAQ needs to estimate a reference threshold $\delta$ and defines the in-distribution context 
\begin{align}\label{eq:in-dis-context}
	\bm{c}_{in} = \left\{\tau_i\left|\sQ(\tau_i)\le \delta, \forall \tau_i \in \bm{c}\right.\right\}.
\end{align}
In this way, IDAQ will perform a two-stage paradigm of online adaptation: (i) a \textit{Reference Stage} to estimate the uncertainty threshold $\delta$ and (ii) an \textit{Iterative Updating Stage} to update the in-distribution context $\bm{c}_{in}$, posterior task belief $q(z|\bm{c}_{in})$, and execution meta-policy $\pi(a|s, z)$.

\textbf{Reference Stage} collects $n_r$ online adaptation episodes $\left\{\tau_i\right\}_{i=1}^{n_r}$ using the prior task distribution $q(z)$ and meta-policy $\pi(a|s, z)$ in a meta-testing task $\kappa_{test}$. IDAQ will calculate the in-distribution confidence of adaptation episodes $\left\{\sQ(\tau_i)\right\}_{i=1}^{n_r}$ and estimate the reference threshold $\delta$ that is the bottom $k\%$-quantile of $\left\{\sQ(\tau_i)\right\}_{i=1}^{n_r}$, where $k$ is a hyperparameter to divide the range of uncertainty of in-distribution episodes. Hence, IDAQ can derive the in-distribution context $\bm{c}_{in}$ and posterior task belief $q(z|\bm{c}_{in})$.

\textbf{Iterative Updating Stage} will update the posterior task belief $q(z|\bm{c}_{in})$ in $n_i$ iterations. In each iteration, IDAQ collects an online adaptation episode $\tau_j$ using the current task belief $q(z|\bm{c}_{in})$ and meta-policy $\pi(a|s, z)$ in $\kappa_{test}$. When the uncertainty of this episode $\sQ(\tau_j)$ is less than the reference threshold $\delta$, IDAQ will update the in-distribution context, i.e., $\bm{c}_{in}\leftarrow\bm{c}_{in}\cup\{\tau_j\}$, and derive the posterior task belief $q(z|\bm{c}_{in})$. The final policy $\pi_{out}(a|s, z)$ is executed with the total in-distribution context $\bm{c}_{in}$.

The overall algorithm of IDAQ is illustrated in Algorithm~\ref{alg:idaq}.

\begin{algorithm}
	\caption{IDAQ: In-Distribution online Adaptation with uncertainty Quantification}\label{alg:idaq}
	\begin{algorithmic}[1]
		\STATE {\bfseries Require:} An offline dataset $\gD^+$, a meta-testing task $\kappa_{test}$, the number of iterations $n_i$, a context-based offline meta-training algorithm $\sA$ (i.e., FOCAL), and an in-distribution uncertainty quantification $\sQ$
		\STATE Offline meta-train a context encoder $q(z|\bm{c})$ and a meta-policy $\pi(a|s, z)$ using an algorithm $\sA$ in a dataset $\gD^+$ \COMMENT{\textbf{\textit{Offline meta-training}}}
		\STATE Perform reference stage of online adaptation and estimate the in-distribution threshold $\delta$ using $\sQ$ \COMMENT{\textbf{\textit{Start online meta-testing}}}
		\STATE Derive the in-distribution context $\bm{c}_{in}$ with Eq. (\ref{eq:in-dis-context}) and posterior task belief $q(z|\bm{c}_{in})$
		\FOR[\textbf{\textit{Iterative updating stage}}]{$t=1\dots n_i$}
		\STATE Collect an online adaptation episode using the posterior task belief $q$ and meta-policy $\pi$ in $\kappa_{test}$
		\STATE Update the in-distribution context $\bm{c}_{in}$ using $\sQ,\delta$ and derive the posterior task belief $q(z|\bm{c}_{in})$
		\ENDFOR
            \STATE {\bfseries Return:} $\pi$, $q(z|\bm{c}_{in})$
	\end{algorithmic}
\end{algorithm}

\vspace{-0.1in}
\subsection{Uncertainty Quantification}
\label{quant}
Uncertainty quantification is a popular tool for empirically measuring the confidence that data is in the distribution of offline RL \cite{yu2020mopo} or noisy oracle \cite{ren2022efficient}. In this subsection, we will analyze three practical uncertainty quantifications to adapt IDAQ to complex domains: \textit{Prediction Error}, \textit{Prediction Variance}, and \textit{Return-based}. The empirical evaluation is deferred to Section \ref{equant}.

To realize the uncertainty quantification of prediction error and prediction variance, we adopt a model-based approach to learn an ensemble of $L$ reward and dynamics models $\left\{r_{\phi_i}(s,a,z), p_{\psi_i}(s,a,z)\right\}_{i=1}^{L}$ according to the latent task embedding $z$. We parameterize them by $\{\phi_i,\psi_i\}_{i=1}^{L}$ and optimize $\left\{r_{\phi_i}, p_{\psi_i}\right\}_{i=1}^{L}$ on the offline multi-task dataset $\gD^+$ by minimizing the MSE loss function during meta-training. Formal loss function is deferred to Appendix \ref{}.

\textbf{Prediction Error} quantifies the model error to estimate the confidence that data is trained during offline meta-training. This metric is also called \textit{"curiosity"}, a popular intrinsic reward in exploration of single-task RL \citep{pathak2017curiosity}, which encourages the agent to visit new areas. In offline meta-RL, we utilize this quantification to filter out out-of-distribution adaptation episodes and denote by
\vspace{-0.03in}
\begin{align}
	\sQ_{PE}(\tau_i, z) =&~ \frac{1}{HL} \sum_{t=0}^{H-1}\sum_{i=1}^{L} \left|r_t-r_{\phi_i}(s_t,a_t,z)\right|  \\
	 &~\qquad\qquad~~~~~+\left\|s_{t+1}-p_{\psi_i}(s_t,a_t,z)\right\|_2, \nonumber
\end{align}

\vspace{-0.1in}
where $z$ is the "task hypothesis" of the episode $\tau_i$ in IDAQ. $\sQ_{PE}$ averages model errors across timesteps and an ensemble. The challenge of $\sQ_{PE}$ is that the hyperparameter $k$ for the reference threshold $\delta$ will be sensitive for different multi-task datasets since the model error of in-distribution episodes can be various.

\textbf{Prediction Variance} captures the epistemic and aleatoric uncertainty of the true models using a bootstrap ensemble \citep{yu2020mopo}. This metric is popular to measure whether data is in the dataset of offline single-task RL \citep{kidambi2020morel}. In offline meta-RL, we denote this quantification by
\vspace{-0.03in}
\begin{align}
	\sQ_{PV}(\tau_i, z) =&~ \frac{1}{H}\sum_{t=0}^{H-1}\max_{i,j}  \left|r_{\phi_i}(s_t,a_t,z)-r_{\phi_j}(s_t,a_t,z)\right|  \nonumber\\
	&~+\left\|p_{\psi_i}(s_t,a_t,z)-p_{\psi_j}(s_t,a_t,z)\right\|_2,
\end{align}
where $z$ is the "task hypothesis" of $\tau_i$. $\sQ_{PV}$ averages the ensemble discrepancy across timesteps. However, $\sQ_{PV}$ cannot handle cases with higher prediction error and lower prediction variance. For example in Figure \ref{fig:MultiTaskDDMExample}, the learned reward model will deterministically output 1 for each action, in which the prediction error is $1-\frac{1}{v}$ with no variance.

\textbf{Return-based} uncertainty quantification is our newly designed metric for offline meta-RL with medium or expert datasets. To address the limitations of prediction error and prediction variance, we utilize a bias of offline RL \citep{fujimoto2019off} that few-shot out-of-distribution episodes generated by an offline-learned meta-policy $\pi$ usually have lower returns since offline meta-training can not well-optimize meta-policies on out-of-distribution states. Its contrapositive statement is that executing $\pi$ with higher returns have a higher probability of being in-distribution and online policy evaluation of $\pi$ presents a good in-distribution confidence:
\vspace{-0.05in}
\begin{align}
\sQ_{RE}\left(\left\{\tau_i\right\}_{i=1}^{n_e}\right) =&~- \frac{1}{n_e}\sum_{i=1}^{n_e}\sum_{t=0}^{H-1} r_t^i,
\end{align}

\vspace{-0.1in}
where $n_e$ is the number of episodes generated by $\pi$ to approximate the online policy evaluation. Note that IDAQ may adopt a conservative (i.e., low) reference threshold $\delta$ to achieve in-distribution online adaptation. In this case, IDAQ may neglect some in-distribution episodes with lower returns. We will argue that, in medium or expert datasets, our method can utilize informative episodes with higher returns to perform task inference. It is an interesting and exciting future direction to differentiate in-distribution episodes with lower return in offline meta-RL with online adaptation. 

